Kinetic Integrals in the Kinetic Theory of dissipative gases

The kinetic theory of gases, including Granular Gases, is based on the Boltzmann equation. Many properties of the gas, from the characteristics of the velocity distribution function to the transport coefficients may be expressed in terms of functions of the collision integral which we call kinetic integrals. Although the evaluation of these functions is conceptually straightforward, technically it is frequently rather cumbersome. We report here a method for the analytical evaluation of kinetic integrals using computer algebra. We apply this method for the computation of some properties of Granular Gases, ranging from the moments of the velocity distribution function to the transport coefficients. For their technical complexity most of these quantities cannot be computed manually.

==> AppenDemomu2.tex <==
%% Created by Maple 7.00 (IBM INTEL LINUX)
%% Source Worksheet: AppenDemomu2.mws
%% Generated: Fri Mar 14 16:12:46 2003
%\documentclass{article}
%\usepackage{maple2e}
 \def\emptyline{\vspace{12pt}}
\DefineParaStyle{Maple Output}
\DefineCharStyle{2D Math}
\DefineCharStyle{2D Output}
%\begin{document}
%\pagestyle{empty}
\begin{maplegroup}
\begin{mapleinput}
\mapleinline{active}{1d}{restart;}{%
}
\end{mapleinput}

\end{maplegroup}
\begin{maplegroup}
\begin{mapleinput}
\mapleinline{active}{1d}{libname:=libname,`/home/kies/KineticIntegral/`:}{%
}
\end{mapleinput}

\end{maplegroup}
\begin{maplegroup}
\begin{mapleinput}
\mapleinline{active}{1d}{with(KineticIntegral);}{%
}
\end{mapleinput}

\mapleresult
\begin{maplelatex}
\mapleinline{inert}{2d}{[DefDimension, DefJ, DefS, KIinit, getJexpr, unDefJ];}{%
\[
[\mathit{DefDimension}, \,\mathit{DefJ}, \,\mathit{DefS}, \,
\mathit{KIinit}, \,\mathit{getJexpr}, \,\mathit{unDefJ}]
\]
%
}
\end{maplelatex}

\end{maplegroup}
\begin{maplegroup}
\begin{mapleinput}
\mapleinline{active}{1d}{KIinit();}{%
}
\end{mapleinput}

\end{maplegroup}
\begin{maplegroup}
\begin{mapleinput}
\mapleinline{active}{1d}{DefDimension(3);}{%
}
\end{mapleinput}

\mapleresult
\begin{maplettyout}
Dimension = 3
\end{maplettyout}

\begin{maplettyout}
Sonine polynomials defined
\end{maplettyout}

\end{maplegroup}
\begin{maplegroup}
\begin{mapleinput}
\mapleinline{active}{1d}{DefJ();}{%
}
\end{mapleinput}

\mapleresult
\begin{maplettyout}
Basic Integrals will be evaluated
\end{maplettyout}

\end{maplegroup}
\begin{maplegroup}
\begin{mapleinput}
\mapleinline{active}{1d}{Expr:=Delta2*(-1/2*(1+a2*(S(2,c1p)+S(2,c2p)))):}{%
}
\end{mapleinput}

\end{maplegroup}
\begin{maplegroup}
\begin{mapleinput}
\mapleinline{active}{1d}{mu2:=getJexpr(0,Expr,0);}{%
}
\end{mapleinput}

\mapleresult
\begin{maplettyout}
expressing 16 terms in form of Basic Integrals
\end{maplettyout}

\begin{maplelatex}
\mapleinline{inert}{2d}{mu2 := -1/16*sqrt(Pi)*sqrt(2)*(epsilon-1)*(1+epsilon)*(16+3*a2);}{%
\[
\mu 2 :=  - {\displaystyle \frac {1}{16}} \,\sqrt{\pi }\,\sqrt{2}
\,(\varepsilon  - 1)\,(1 + \varepsilon )\,(16 + 3\,\mathit{a2})
\]
%
}
\end{maplelatex}

\end{maplegroup}
%\end{document}
%% End of Maple 7.00 Output

